Projecting the Impact of Covid-19 Variants and Vaccination Strategies in Disease Transmission using a Multilayer Network Model in Costa Rica

For countries starting to receive steady supplies of vaccines against SARS-CoV-2, the course of Covid-19 for the following months will be determined by the emergence of new variants and successful roll-out of vaccination campaigns. To anticipate this scenario, we used a multilayer network model developed to forecast the transmission dynamics of Covid-19 in Costa Rica, and to estimate the impact of the introduction of the Delta variant in the country, under two plausible vaccination scenarios, one sustaining Costa Rica's July 2021 vaccination pace of 30,000 doses per day and with high acceptance from the population and another with declining vaccination pace to 13,000 doses per day and with lower acceptance. Results suggest that the introduction and gradual dominance of the Delta variant would increase Covid-19 hospitalizations and ICU admissions between $35\%$ and $33.25\%$, from August 2021 to December 2021, depending on vaccine administration and acceptance. In the presence of the Delta variant, new Covid-19 hospitalizations and ICU admission would experience an average increase of $24.26\%$ and $27.19\%$ respectively in the same period if the vaccination pace drops. Our results can help decision-makers better prepare for the COVID-19 pandemic in the months to come.

==> bibliography.tex <==
\begin{thebibliography}{10}
\urlstyle{rm}
\expandafter\ifx\csname url\endcsname\relax
  \def\url#1{\texttt{#1}}\fi
\expandafter\ifx\csname urlprefix\endcsname\relax\def\urlprefix{URL }\fi
\expandafter\ifx\csname doiprefix\endcsname\relax\def\doiprefix{DOI: }\fi
\providecommand{\bibinfo}[2]{#2}
\providecommand{\eprint}[2][]{\url{#2}}

\bibitem{kim2020covid}
\bibinfo{author}{Kim, Y.~C.}, \bibinfo{author}{Dema, B.} \&
  \bibinfo{author}{Reyes-Sandoval, A.}
\newblock \bibinfo{journal}{\bibinfo{title}{Covid-19 vaccines: breaking record
  times to first-in-human trials}}.
\newblock {\emph{\JournalTitle{NPJ Vaccines}}} \textbf{\bibinfo{volume}{5}},
  \bibinfo{pages}{1--3}, \doiprefix\url{10.1038/s41541-020-0188-3}
  (\bibinfo{year}{2020}).

\bibitem{li2021comprehensive}
\bibinfo{author}{Li, Y.} \emph{et~al.}
\newblock \bibinfo{journal}{\bibinfo{title}{A comprehensive review of the
  global efforts on \uppercase{COVID}-19 vaccine development}}.
\newblock {\emph{\JournalTitle{ACS Cent. Sci.}}} \textbf{\bibinfo{volume}{7}},
  \bibinfo{pages}{512--533}, \doiprefix\url{10.1021/acscentsci.1c00120}
  (\bibinfo{year}{2021}).

\bibitem{wang2020genetic}
\bibinfo{author}{Wang, H.} \emph{et~al.}
\newblock \bibinfo{journal}{\bibinfo{title}{The genetic sequence, origin, and
  diagnosis of \uppercase{SARS}-\uppercase{C}o\uppercase{V}-2}}.
\newblock {\emph{\JournalTitle{Europ. J. Clin. Microbiol. Infect. Dis.}}}
  \textbf{\bibinfo{volume}{39}}, \bibinfo{pages}{1629--1635},
  \doiprefix\url{10.1007/s10096-020-03899-4} (\bibinfo{year}{2020}).

\bibitem{Vaccines57:online}
\bibinfo{author}{Basta, N.} \& \bibinfo{author}{Moodie, E.}
\newblock \bibinfo{title}{\uppercase{COVID}-19 vaccine development and
  approvals tracker}.
\newblock
  \bibinfo{howpublished}{\url{https://covid19.trackvaccines.org/vaccines/approved/\#vaccine-list}}
  (\bibinfo{year}{2021}).

\bibitem{COVID19v90:online}
\bibinfo{author}{WHO}.
\newblock \bibinfo{title}{\uppercase{COVID}-19 vaccine tracker and landscape}.
\newblock
  \bibinfo{howpublished}{\url{https://www.who.int/publications/m/item/draft-landscape-of-covid-19-candidate-vaccines}}
  (\bibinfo{year}{2021}).

\bibitem{wouters2021challenges}
\bibinfo{author}{Wouters, O.~J.} \emph{et~al.}
\newblock \bibinfo{journal}{\bibinfo{title}{Challenges in ensuring global
  access to \uppercase{COVID}-19 vaccines: production, affordability,
  allocation, and deployment}}.
\newblock {\emph{\JournalTitle{The Lancet}}} \textbf{\bibinfo{volume}{397}},
  \bibinfo{pages}{10278--1034}, \doiprefix\url{10.1016/S0140-6736(21)00306-8}
  (\bibinfo{year}{2021}).

\bibitem{acharya2021access}
\bibinfo{author}{Acharya, K.~P.}, \bibinfo{author}{Ghimire, T.~R.} \&
  \bibinfo{author}{Subramanya, S.~H.}
\newblock \bibinfo{journal}{\bibinfo{title}{Access to and equitable
  distribution of \uppercase{COVID}-19 vaccine in low-income countries}}.
\newblock {\emph{\JournalTitle{NPJ Vaccines}}} \textbf{\bibinfo{volume}{6}},
  \bibinfo{pages}{54}, \doiprefix\url{10.1038/s41541-021-00323-6}
  (\bibinfo{year}{2021}).

\bibitem{arce2021covid}
\bibinfo{author}{Arce, J. S.~S.} \emph{et~al.}
\newblock \bibinfo{journal}{\bibinfo{title}{\uppercase{COVID}-19 vaccine
  acceptance and hesitancy in low-and middle-income countries}}.
\newblock {\emph{\JournalTitle{Nat. Med.}}} \textbf{\bibinfo{volume}{27}},
  \bibinfo{pages}{1385--1394}, \doiprefix\url{10.1038/s41591-021-01454-y}
  (\bibinfo{year}{2021}).

\bibitem{sallam2021covid}
\bibinfo{author}{Sallam, M.}
\newblock \bibinfo{journal}{\bibinfo{title}{\uppercase{COVID}-19 vaccine
  hesitancy worldwide: a concise systematic review of vaccine acceptance
  rates}}.
\newblock {\emph{\JournalTitle{Vaccines}}} \textbf{\bibinfo{volume}{9}},
  \bibinfo{pages}{160}, \doiprefix\url{10.3390/vaccines9020160}
  (\bibinfo{year}{2021}).

\bibitem{abdool2021new}
\bibinfo{author}{Abdool~Karim, S.~S.} \& \bibinfo{author}{de~Oliveira, T.}
\newblock \bibinfo{journal}{\bibinfo{title}{New
  \uppercase{SARS}-\uppercase{C}o\uppercase{V}-2 variants—clinical, public
  health, and vaccine implications}}.
\newblock {\emph{\JournalTitle{N. Engl. J. Med.}}}
  \textbf{\bibinfo{volume}{384}}, \bibinfo{pages}{1866--1868},
  \doiprefix\url{10.1056/NEJMc2100362} (\bibinfo{year}{2021}).

\bibitem{walensky2021sars}
\bibinfo{author}{Walensky, R.~P.}, \bibinfo{author}{Walke, H.~T.} \&
  \bibinfo{author}{Fauci, A.~S.}
\newblock
  \bibinfo{journal}{\bibinfo{title}{\uppercase{SARS}-\uppercase{C}o\uppercase{V}-2
  variants of concern in the united states—challenges and opportunities}}.
\newblock {\emph{\JournalTitle{Jama}}} \textbf{\bibinfo{volume}{325}},
  \bibinfo{pages}{1037--1038}, \doiprefix\url{10.1001/jama.2021.2294}
  (\bibinfo{year}{2021}).

\bibitem{Tracking0:online}
\bibinfo{author}{WHO}.
\newblock \bibinfo{title}{Tracking
  \uppercase{SARS}-\uppercase{C}o\uppercase{V}-2 variants}.
\newblock
  \bibinfo{howpublished}{\url{https://www.who.int/en/activities/tracking-SARS-CoV-2-variants}}
  (\bibinfo{year}{20021}).

\bibitem{davies2021estimated}
\bibinfo{author}{Davies, N.~G.} \emph{et~al.}
\newblock \bibinfo{journal}{\bibinfo{title}{Estimated transmissibility and
  impact of \uppercase{SARS}-\uppercase{C}o\uppercase{V}-2 lineage
  \uppercase{B}.1.1.7 in \uppercase{E}ngland}}.
\newblock {\emph{\JournalTitle{Science}}} \textbf{\bibinfo{volume}{372}},
  \bibinfo{pages}{eabg3055}, \doiprefix\url{10.1126/science.abg3055}
  (\bibinfo{year}{2021}).

\bibitem{nyberg2021risk}
\bibinfo{author}{Nyberg, T.} \emph{et~al.}
\newblock \bibinfo{journal}{\bibinfo{title}{Risk of hospital admission for
  patients with \uppercase{SARS}-\uppercase{C}o\uppercase{V}-2 variant
  \uppercase{B}.1.1.7: cohort analysis}}.
\newblock {\emph{\JournalTitle{BMJ}}} \textbf{\bibinfo{volume}{373}},
  \bibinfo{pages}{n1412}, \doiprefix\url{10.1136/bmj.n1412}
  (\bibinfo{year}{2021}).

\bibitem{challen2021risk}
\bibinfo{author}{Challen, R.} \emph{et~al.}
\newblock \bibinfo{journal}{\bibinfo{title}{Risk of mortality in patients
  infected with \uppercase{SARS}-\uppercase{C}o\uppercase{V}-2 variant of
  concern 202012/1: matched cohort study}}.
\newblock {\emph{\JournalTitle{BMJ}}} \textbf{\bibinfo{volume}{372}},
  \bibinfo{pages}{n579}, \doiprefix\url{10.1136/bmj.n579}
  (\bibinfo{year}{2021}).

\bibitem{bernal2021delta}
\bibinfo{author}{Bernal, J.~L.} \emph{et~al.}
\newblock \bibinfo{journal}{\bibinfo{title}{Effectiveness of
  \uppercase{COVID}-19 vaccines against the \uppercase{B}.1.617.2 variant}}.
\newblock {\emph{\JournalTitle{N. Engl. J. Med.}}}
  \textbf{\bibinfo{volume}{385}}, \bibinfo{pages}{385--594},
  \doiprefix\url{10.1056/NEJMoa2108891} (\bibinfo{year}{2021}).

\bibitem{COVID19v12:online}
\bibinfo{author}{England, P.~H.}
\newblock \bibinfo{title}{Covid-19 vaccine surveillance report - week 31}.
\newblock
  \bibinfo{howpublished}{\url{https://assets.publishing.service.gov.uk/government/uploads/system/uploads/attachment_data/file/1008919/Vaccine_surveillance_report_-_week_31.pdf}}
  (\bibinfo{year}{2021}).

\bibitem{callaway2021covid}
\bibinfo{author}{Callaway, E.}
\newblock \bibinfo{journal}{\bibinfo{title}{\uppercase{COVID} vaccine boosters:
  the most important questions.}}
\newblock {\emph{\JournalTitle{Nature}}} \textbf{\bibinfo{volume}{596}},
  \bibinfo{pages}{178--180}, \doiprefix\url{10.1038/d41586-021-02158-6}
  (\bibinfo{year}{2021}).

\bibitem{COVIDvar91:online}
\bibinfo{author}{UN}.
\newblock \bibinfo{title}{\uppercase{COVID} variants ‘winning the race
  against vaccines’ warns \uppercase{WHO} chief | | \uppercase{UN} news}.
\newblock
  \bibinfo{howpublished}{\url{https://news.un.org/en/story/2021/07/1095432}}
  (\bibinfo{year}{2021}).

\bibitem{loomba2021measuring}
\bibinfo{author}{Loomba, S.}, \bibinfo{author}{de~Figueiredo, A.},
  \bibinfo{author}{Piatek, S.~J.}, \bibinfo{author}{de~Graaf, K.} \&
  \bibinfo{author}{Larson, H.~J.}
\newblock \bibinfo{journal}{\bibinfo{title}{Measuring the impact of
  \uppercase{COVID}-19 vaccine misinformation on vaccination intent in the
  \uppercase{UK} and \uppercase{USA}}}.
\newblock {\emph{\JournalTitle{Nat. Hum. Behav.}}}
  \textbf{\bibinfo{volume}{5}}, \bibinfo{pages}{337--348},
  \doiprefix\url{10.1038/s41562-021-01056-1} (\bibinfo{year}{2021}).

\bibitem{van2021inoculating}
\bibinfo{author}{van~der Linden, S.}, \bibinfo{author}{Dixon, G.},
  \bibinfo{author}{Clarke, C.} \& \bibinfo{author}{Cook, J.}
\newblock \bibinfo{journal}{\bibinfo{title}{Inoculating against
  \uppercase{COVID}-19 vaccine misinformation}}.
\newblock {\emph{\JournalTitle{EClinicalMedicine}}}
  \textbf{\bibinfo{volume}{33}}, \doiprefix\url{10.1016/j.eclinm.2021.100772}
  (\bibinfo{year}{2021}).

\bibitem{moore2021modelling}
\bibinfo{author}{Moore, S.}, \bibinfo{author}{Hill, E.~M.},
  \bibinfo{author}{Dyson, L.}, \bibinfo{author}{Tildesley, M.~J.} \&
  \bibinfo{author}{Keeling, M.~J.}
\newblock \bibinfo{journal}{\bibinfo{title}{Modelling optimal vaccination
  strategy for \uppercase{SARS}-\uppercase{C}o\uppercase{V}-2 in the
  \uppercase{UK}}}.
\newblock {\emph{\JournalTitle{PLoS Comput. Biol.}}}
  \textbf{\bibinfo{volume}{17}}, \bibinfo{pages}{e1008849},
  \doiprefix\url{10.1371/journal.pcbi.1008849} (\bibinfo{year}{2021}).

\bibitem{matrajt2021optimizing}
\bibinfo{author}{Matrajt, L.} \emph{et~al.}
\newblock \bibinfo{journal}{\bibinfo{title}{Optimizing vaccine allocation for
  \uppercase{COVID}-19 vaccines shows the potential role of single-dose
  vaccination}}.
\newblock {\emph{\JournalTitle{Nat. Commun.}}} \textbf{\bibinfo{volume}{12}},
  \bibinfo{pages}{3449}, \doiprefix\url{10.1038/s41467-021-23761-1}
  (\bibinfo{year}{2021}).

\bibitem{paltiel2021speed}
\bibinfo{author}{Paltiel, A.~D.}, \bibinfo{author}{Zheng, A.} \&
  \bibinfo{author}{Schwartz, J.~L.}
\newblock \bibinfo{journal}{\bibinfo{title}{Speed versus efficacy: quantifying
  potential tradeoffs in \uppercase{COVID}-19 vaccine deployment}}.
\newblock {\emph{\JournalTitle{Ann. Intern. Med.}}}
  \textbf{\bibinfo{volume}{174}}, \bibinfo{pages}{568--570},
  \doiprefix\url{10.7326/M20-7866} (\bibinfo{year}{2021}).

\bibitem{coudeville2021potential}
\bibinfo{author}{Coudeville, L.}, \bibinfo{author}{Jollivet, O.},
  \bibinfo{author}{Mah{\'e}, C.}, \bibinfo{author}{Chaves, S.} \&
  \bibinfo{author}{Gomez, G.~B.}
\newblock \bibinfo{journal}{\bibinfo{title}{Potential impact of introducing
  vaccines against \uppercase{COVID}-19 under supply and uptake constraints in
  \uppercase{F}rance: A modelling study}}.
\newblock {\emph{\JournalTitle{Plos One}}} \textbf{\bibinfo{volume}{16}},
  \bibinfo{pages}{e0250797}, \doiprefix\url{10.1371/journal.pone.0250797}
  (\bibinfo{year}{2021}).

\bibitem{romero2021public}
\bibinfo{author}{Romero-Brufau, S.} \emph{et~al.}
\newblock \bibinfo{journal}{\bibinfo{title}{Public health impact of delaying
  second dose of \uppercase{BNT}162b2 or m\uppercase{RNA}-1273
  \uppercase{COVID}-19 vaccine: simulation agent based modeling study}}.
\newblock {\emph{\JournalTitle{BMJ}}} \textbf{\bibinfo{volume}{373}},
  \bibinfo{pages}{n1334}, \doiprefix\url{10.1136/bmj.n1334}
  (\bibinfo{year}{2021}).

\bibitem{tetteh2020covid}
\bibinfo{author}{Tetteh, J.~N.}, \bibinfo{author}{Vargas, E. A.~H.}
  \emph{et~al.}
\newblock \bibinfo{journal}{\bibinfo{title}{\uppercase{COVID}-19 network model
  to evaluate vaccine strategies towards herd immunity}}.
\newblock {\emph{\JournalTitle{medRxiv}}}
  \doiprefix\url{10.1101/2020.12.22.20248693} (\bibinfo{year}{2020}).

\bibitem{giordano2021modeling}
\bibinfo{author}{Giordano, G.} \emph{et~al.}
\newblock \bibinfo{journal}{\bibinfo{title}{Modeling vaccination rollouts,
  \uppercase{SARS}-\uppercase{C}o\uppercase{V}-2 variants and the requirement
  for non-pharmaceutical interventions in \uppercase{I}taly}}.
\newblock {\emph{\JournalTitle{Nat. Med.}}} \textbf{\bibinfo{volume}{27}},
  \bibinfo{pages}{993--998}, \doiprefix\url{10.1038/s41591-021-01334-5}
  (\bibinfo{year}{2021}).

\bibitem{usherwood2021model}
\bibinfo{author}{Usherwood, T.}, \bibinfo{author}{LaJoie, Z.} \&
  \bibinfo{author}{Srivastava, V.}
\newblock \bibinfo{journal}{\bibinfo{title}{A model and predictions for
  \uppercase{COVID}-19 considering population behavior and vaccination}}.
\newblock {\emph{\JournalTitle{Sci. Rep.}}} \textbf{\bibinfo{volume}{11}},
  \bibinfo{pages}{12051}, \doiprefix\url{10.1038/s41598-021-91514-7}
  (\bibinfo{year}{2021}).

\bibitem{rella2021rates}
\bibinfo{author}{Rella, S.~A.}, \bibinfo{author}{Kulikova, Y.~A.},
  \bibinfo{author}{Dermitzakis, E.~T.} \& \bibinfo{author}{Kondrashov, F.~A.}
\newblock \bibinfo{journal}{\bibinfo{title}{Rates of
  \uppercase{SARS}-\uppercase{C}o\uppercase{V}-2 transmission and vaccination
  impact the fate of vaccine-resistant strains}}.
\newblock {\emph{\JournalTitle{Sci. Rep.}}} \textbf{\bibinfo{volume}{11}},
  \bibinfo{pages}{15729}, \doiprefix\url{10.1038/s41598-021-95025-3}
  (\bibinfo{year}{2021}).

\bibitem{caldwella2021vaccines}
\bibinfo{author}{Caldwella, J.~M.} \emph{et~al.}
\newblock \bibinfo{journal}{\bibinfo{title}{Vaccines and variants: modelling
  insights into emerging issues in \uppercase{COVID}-19 epidemiology}}.
\newblock {\emph{\JournalTitle{Paediatr. Respir. Rev.}}}
  \bibinfo{pages}{S1526--0542}, \doiprefix\url{10.1016/j.prrv.2021.07.002}
  (\bibinfo{year}{2021}).

\bibitem{Lineamie32:online}
\bibinfo{author}{MINSA}.
\newblock \bibinfo{title}{Situaci\'on nacional \uppercase{C}ovid-19}.
\newblock
  \bibinfo{howpublished}{\url{https://www.ministeriodesalud.go.cr/index.php/centro-de-prensa/noticias/741-noticias-2020/1532-lineamientos-nacionales-para-la-vigilancia-de-la-infeccion-por-coronavirus-2019-ncov}}
  (\bibinfo{year}{2021}).

\bibitem{parry2021extended}
\bibinfo{author}{Parry, H.~M.} \emph{et~al.}
\newblock \bibinfo{journal}{\bibinfo{title}{Extended interval
  \uppercase{BNT}162b2 vaccination enhances peak antibody generation in older
  people}}.
\newblock {\emph{\JournalTitle{MedRxiv}}}
  \doiprefix\url{10.1101/2021.05.15.21257017} (\bibinfo{year}{2021}).

\bibitem{WHOCoron71:online}
\bibinfo{author}{WHO}.
\newblock \bibinfo{title}{Who coronavirus (\uppercase{COVID}-19) dashboard |
  \uppercase{WHO} coronavirus (\uppercase{COVID}-19) dashboard with vaccination
  data}.
\newblock \bibinfo{howpublished}{\url{https://covid19.who.int/}}
  (\bibinfo{year}{2021}).

\bibitem{Bienveni11:online}
\bibinfo{author}{INEC}.
\newblock \bibinfo{title}{Instituto \uppercase{N}acional de
  \uppercase{E}stad\'istica y \uppercase{C}enso}.
\newblock \bibinfo{howpublished}{\url{https://www.inec.cr/}}
  (\bibinfo{year}{2021}).

\bibitem{ccstarifa}
\bibinfo{author}{CCSS}.
\newblock \bibinfo{title}{Modelo tarifario seguro de salud.
  \uppercase{D}irecci\'on financiera contable \'area contabilidad de costos
  sub\'area contabilidad de costos hospitalarios. \uppercase{V}igencia a partir
  del 01 de julio del 2020} (\bibinfo{year}{2020}).

\bibitem{COVID19C0:online}
\bibinfo{author}{CCSS}.
\newblock \bibinfo{title}{\uppercase{COVID}-19 \uppercase{CCSS} | vacunación}.
\newblock
  \bibinfo{howpublished}{\url{https://www.ccss.sa.cr/web/coronavirus/vacunacion}}
  (\bibinfo{year}{2021}).

\bibitem{solis2021covid}
\bibinfo{author}{Sol{\'\i}s~Arce, J.~S.} \emph{et~al.}
\newblock \bibinfo{journal}{\bibinfo{title}{\uppercase{COVID}-19 vaccine
  acceptance and hesitancy in low-and middle-income countries}}.
\newblock {\emph{\JournalTitle{Nat. Med.}}} \textbf{\bibinfo{volume}{27}},
  \bibinfo{pages}{1385--1394}, \doiprefix\url{10.1038/s41591-021-01454-y}
  (\bibinfo{year}{2021}).

\bibitem{calvo2021multilayer}
\bibinfo{author}{Calvo, J.~G.}, \bibinfo{author}{Sanchez, F.},
  \bibinfo{author}{Barboza, L.~A.}, \bibinfo{author}{Garc{\'\i}a, Y.~E.} \&
  \bibinfo{author}{V{\'a}squez, P.}
\newblock \bibinfo{journal}{\bibinfo{title}{A multilayer network model
  implementation for \uppercase{C}ovid-19}}.
\newblock {\emph{\JournalTitle{arXiv preprint arXiv:2103.08843}}}
  (\bibinfo{year}{2021}).

\bibitem{kang2020age}
\bibinfo{author}{Kang, S.-J.} \& \bibinfo{author}{Jung, S.~I.}
\newblock \bibinfo{journal}{\bibinfo{title}{Age-related morbidity and mortality
  among patients with \uppercase{COVID}-19}}.
\newblock {\emph{\JournalTitle{Infect. Chemother.}}}
  \textbf{\bibinfo{volume}{52}}, \bibinfo{pages}{154--164},
  \doiprefix\url{10.3947/ic.2020.52.2.154} (\bibinfo{year}{2020}).

\bibitem{bernal2021effectiveness}
\bibinfo{author}{Bernal, J.~L.} \emph{et~al.}
\newblock \bibinfo{journal}{\bibinfo{title}{Effectiveness of the
  \uppercase{P}fizer-\uppercase{B}io \uppercase{NT}ech and
  \uppercase{O}xford-\uppercase{A}stra\uppercase{Z}eneca vaccines on
  \uppercase{C}ovid-19 related symptoms, hospital admissions, and mortality in
  older adults in \uppercase{E}ngland: test negative case-control study}}.
\newblock {\emph{\JournalTitle{BMJ}}} \textbf{\bibinfo{volume}{373}},
  \bibinfo{pages}{n1088}, \doiprefix\url{10.1136/bmj.n1088}
  (\bibinfo{year}{2021}).

\bibitem{COVID19v59:online}
\bibinfo{author}{England, P.~H.}
\newblock \bibinfo{title}{\uppercase{COVID}-19 vaccine surveillance report -
  week 33}.
\newblock
  \bibinfo{howpublished}{\url{https://assets.publishing.service.gov.uk/government/uploads/system/uploads/attachment_data/file/1012420/Vaccine_surveillance_report_-_week_33.pdf}}
  (\bibinfo{year}{2021}).

\bibitem{Matlab}
\bibinfo{author}{MATLAB}.
\newblock \emph{\bibinfo{title}{version 9.8.0 (R2020a)}}
  (\bibinfo{publisher}{The MathWorks Inc.}, \bibinfo{address}{Natick,
  Massachusetts}, \bibinfo{year}{2020}).

\bibitem{van2021covid}
\bibinfo{author}{van Oosterhout, C.}, \bibinfo{author}{Hall, N.},
  \bibinfo{author}{Ly, H.} \& \bibinfo{author}{Tyler, K.~M.}
\newblock \bibinfo{title}{Covid-19 evolution during the pandemic--implications
  of new \uppercase{SARS}-\uppercase{C}o\uppercase{V}-2 variants on disease
  control and public health policies},
  \doiprefix\url{10.1080/21505594.2021.1877066} (\bibinfo{year}{2021}).

\bibitem{borchering2021modeling}
\bibinfo{author}{Borchering, R.~K.} \emph{et~al.}
\newblock \bibinfo{journal}{\bibinfo{title}{Modeling of future
  \uppercase{COVID}-19 cases, hospitalizations, and deaths, by vaccination
  rates and nonpharmaceutical intervention scenarios—united states,
  april--september 2021}}.
\newblock {\emph{\JournalTitle{MMWR Morb Mortal Wkly Rep}}}
  \textbf{\bibinfo{volume}{70}}, \bibinfo{pages}{719--724},
  \doiprefix\url{10.15585/mmwr.mm7019e3} (\bibinfo{year}{2021}).

\bibitem{sah2021accelerated}
\bibinfo{author}{Sah, P.} \emph{et~al.}
\newblock \bibinfo{journal}{\bibinfo{title}{Accelerated vaccine rollout is
  imperative to mitigate highly transmissible \uppercase{COVID}-19 variants}}.
\newblock {\emph{\JournalTitle{EClinicalMedicine}}}
  \textbf{\bibinfo{volume}{35}}, \bibinfo{pages}{100865},
  \doiprefix\url{10.1016/j.eclinm.2021.100865} (\bibinfo{year}{2021}).

\bibitem{alagoz2021impact}
\bibinfo{author}{Alagoz, O.} \emph{et~al.}
\newblock \bibinfo{journal}{\bibinfo{title}{The impact of vaccination to
  control \uppercase{COVID}-19 burden in the \uppercase{U}nited
  \uppercase{S}tates: A simulation modeling approach}}.
\newblock {\emph{\JournalTitle{Plos One}}} \textbf{\bibinfo{volume}{16}},
  \bibinfo{pages}{e0254456}, \doiprefix\url{10.1371/journal.pone.0254456}
  (\bibinfo{year}{2021}).

\bibitem{Vaccinei55:online}
\bibinfo{author}{WHO}.
\newblock \bibinfo{title}{Vaccine inequity undermining global economic
  recovery}.
\newblock
  \bibinfo{howpublished}{\url{https://www.who.int/news/item/22-07-2021-vaccine-inequity-undermining-global-economic-recovery}}
  (\bibinfo{year}{2021}).

\bibitem{world2020pandemic}
\bibinfo{author}{WHO}.
\newblock \bibinfo{title}{Pandemic fatigue: reinvigorating the public to
  prevent \uppercase{C}ovid-19: policy framework for supporting pandemic
  prevention and management: revised version \uppercase{N}ovember 2020}.
\newblock \bibinfo{type}{Tech. Rep.}, \bibinfo{institution}{World Health
  Organization. Regional Office for Europe} (\bibinfo{year}{2020}).

\bibitem{saludpdf2:online}
\bibinfo{author}{OCDE}.
\newblock \bibinfo{title}{Estudios de la ocde sobre los sistemas de salud:
  \uppercase{C}osta \uppercase{R}ica}.
\newblock
  \bibinfo{howpublished}{\url{https://www.comex.go.cr/media/8460/salud.pdf}}
  (\bibinfo{year}{2017}).

\bibitem{LibroPer43:online}
\bibinfo{author}{WHO/PAHO}.
\newblock \bibinfo{title}{Perfil del sistema y servicio de salud de
  \uppercase{C}osta \uppercase{R}ica}.
\newblock
  \bibinfo{howpublished}{\url{file:///C:/Users/Lenovo/Downloads/OPSCRI19001_spa.pdf}}
  (\bibinfo{year}{2018}).

\bibitem{657pdf6:online}
\bibinfo{author}{CCSS}.
\newblock \bibinfo{title}{Medidas para mitigar el impacto financiero de la
  pandemia del \uppercase{C}ovid-19, para los años 2021-2022}.
\newblock
  \bibinfo{howpublished}{\url{https://www.ccss.sa.cr/web/coronavirus/assets/materiales/personal/lineamientos/657.pdf}}
  (\bibinfo{year}{2021}).

\bibitem{office2020coronavirus}
\bibinfo{author}{ONS}.
\newblock \bibinfo{title}{Coronavirus and the social impacts on
  \uppercase{G}reat \uppercase{B}ritain}.
\newblock
  \bibinfo{howpublished}{\url{https://www.ons.gov.uk/peoplepopulationandcommunity/healthandsocialcare/healthandwellbeing/datasets/coronavirusandthesocialimpactsongreatbritaindata}}
  (\bibinfo{year}{2020}).

\bibitem{keeling2011effects}
\bibinfo{author}{Keeling, M.~J.}, \bibinfo{author}{Newman, M.},
  \bibinfo{author}{Barab{\'a}si, A.-L.} \& \bibinfo{author}{Watts, D.~J.}
\newblock \bibinfo{title}{The effects of local spatial structure on
  epidemiological invasions}.
\newblock In \emph{\bibinfo{booktitle}{The Structure and Dynamics of
  Networks}}, \bibinfo{pages}{480--488} (\bibinfo{publisher}{Princeton
  University Press}, \bibinfo{year}{2011}).

\bibitem{bish2011factors}
\bibinfo{author}{Bish, A.}, \bibinfo{author}{Yardley, L.},
  \bibinfo{author}{Nicoll, A.} \& \bibinfo{author}{Michie, S.}
\newblock \bibinfo{journal}{\bibinfo{title}{Factors associated with uptake of
  vaccination against pandemic influenza: a systematic review}}.
\newblock {\emph{\JournalTitle{Vaccine}}} \textbf{\bibinfo{volume}{29}},
  \bibinfo{pages}{6472--6484}, \doiprefix\url{10.1016/j.vaccine.2011.06.107}
  (\bibinfo{year}{2011}).

\bibitem{polack2020safety}
\bibinfo{author}{Polack, F.~P.} \emph{et~al.}
\newblock \bibinfo{journal}{\bibinfo{title}{Safety and efficacy of the
  \uppercase{BNT}162b2 m\uppercase{RNA} \uppercase{C}ovid-19 vaccine}}.
\newblock {\emph{\JournalTitle{N. Engl. J. Med.}}}
  \textbf{\bibinfo{volume}{383}}, \bibinfo{pages}{2603--2615},
  \doiprefix\url{10.1056/NEJMoa2034577} (\bibinfo{year}{2020}).

\bibitem{keehner2021sars}
\bibinfo{author}{Keehner, J.} \emph{et~al.}
\newblock
  \bibinfo{journal}{\bibinfo{title}{\uppercase{SARS}-\uppercase{C}o\uppercase{V}-2
  infection after vaccination in health care workers in
  \uppercase{C}alifornia}}.
\newblock {\emph{\JournalTitle{N. Engl. J. Med.}}}
  \textbf{\bibinfo{volume}{384}}, \bibinfo{pages}{1774--1775},
  \doiprefix\url{10.1056/NEJMc2101927} (\bibinfo{year}{2021}).

\bibitem{10.1093/cid/ciab554}
\bibinfo{author}{Jacobson, K.~B.} \emph{et~al.}
\newblock \bibinfo{journal}{\bibinfo{title}{{Post-Vaccination Severe Acute
  Respiratory Syndrome Coronavirus 2
  (\uppercase{SARS}-\uppercase{C}o\uppercase{V}-2) Infections and Incidence of
  the Presumptive \uppercase{B}.1.427/\uppercase{B}.1.429 Variant Among
  Healthcare Personnel at a Northern California Academic Medical Center}}}.
\newblock {\emph{\JournalTitle{Clin. Infect. Dis.}}}
  \doiprefix\url{10.1093/cid/ciab554} (\bibinfo{year}{2021}).

\end{thebibliography}
